Wafer2Spike: Spiking Neural Network for Wafer Map Pattern Classification

In integrated circuit design, the analysis of wafer map patterns is critical to improve yield and detect manufacturing issues. We develop Wafer2Spike, an architecture for wafer map pattern classification using a spiking neural network (SNN), and demonstrate that a well-trained SNN achieves superior performance compared to deep neural network-based solutions. Wafer2Spike achieves an average classification accuracy of 98\% on the WM-811k wafer benchmark dataset. It is also superior to existing approaches for classifying defect patterns that are underrepresented in the original dataset. Wafer2Spike achieves this improved precision with great computational efficiency.

==> sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}
%Learning techniques for wafer map pattern analysis can be grouped into unsupervised and supervised categories. 

\emph{Unsupervised learning methods} have been developed to group wafer maps by their defect patterns after which test engineers manually categorize each map based on its specific defects~\cite{chien2013system, alawieh2016identifying, alawieh2017identifying}. Nero et al. introduced an unsupervised technique employing generative adversarial networks to train recognizers for wafer map pattern identification, although this approach requires considerable manual adjustments throughout the learning phase~\cite{nero2018concept}.

\emph{Supervised learning} with the K-nearest neighbor algorithm has been applied to classify defective wafer maps by analyzing spatial signature features~\cite{tobin1997automatic,karnowski1999application}. Support Vector Machines (SVMs) have been employed, training the system with features obtained from radon and geometric transformations~\cite{wu2014wafer, fan2016wafer}. 
More recently, CNNs, with their ability to learn features from raw data, have been used to identify wafer map patterns with very good classification accuracy~\cite{alawieh2020wafer, tsai2020light, du2020wafer,}. 

Alawieh et al. have developed a CNN model that includes a reject option to reduce misclassification risk~\cite{alawieh2020wafer}. The model contains three convolutional, one fully connected, and output layers. Genssler et al. use brain-inspired hyperdimensional computing to first transform wafer map features into hypervectors and then use a simple two-layer perceptron model (MLP) for classification~\cite{genssler2021brain}. Their MC32+MLP model uses 32 hypervectors per class, which are then processed by the MLP to classify the defects. Tsai et al. adapt the MobileNetV1 architecture to develop a classifier with a deep detachable convolution architecture, named Defect-Map Classification (DMC1)~\cite{tsai2020light}. This model comprises ten convolutional layers, one fully connected layer, and an output layer. Finally, Liao et al. develop a multi-task learning framework called $P^2$-Net, which uses both pattern- and pixel-level information from wafer maps to improve classification accuracy~\cite{liao2022wafer}. It uses a three-layer neural network to identify defect patterns across the entire wafer map, complemented by a decoder network that classifies each pixel of the wafer map individually.






==> sections/unused.tex <==
%Deep Neural Networks (DNNs), inspired by the biological neuro-synaptic structure have shown significant effectiveness in classifying wafer map patterns\cite{lecun2015deep, alawieh2020wafer, wu2014wafer, genssler2021brain, tsai2020light, liao2022wafer}. This efficiency is attributed to their capacity for learning directly from raw data and exhibiting strong generalization ability \cite{zhang2021understanding}. However, with their remarkable capabilities, the high energy costs associated with DNN inference \cite{dong2017more} pose a significant challenge. This limitation is particularly problematic when deploying DNNs in real-time systems or on devices constrained by available energy resources. The intensive computational requirements of DNNs demand considerable energy, which can hinder their  application in environments where power availability is limited or the cost of energy consumption is a critical factor.


%For instance, training a massive transformer-based neural network model requires approximately 190,000 kWh of energy \cite{budennyy2022eco2ai, anthony2020carbontracker, dhar2020carbon}.
%In contrast, the human brain, with its complex capabilities including perception, recognition, reasoning, control, and movement, operates on a mere 20 W of power \cite{cox2014neural}. 
